Formality of derived intersections and the orbifold HKR isomorphism

We study when the derived intersection of two smooth subvarieties of a smooth variety is formal. As a consequence we obtain a derived base change theorem for non-transversal intersections. We also obtain applications to the study of the derived fixed locus of a finite group action and argue that for a global quotient orbifold the exponential map is an isomorphism between the Lie algebra of the free loop space and the loop space itself. This allows us to give new proofs of the HKR decomposition of orbifold Hochschild (co)homology into twisted sectors.

==> pagesize.tex <==
\headheight=8pt     \topmargin=0pt
\textheight=624pt   \textwidth=448pt
\oddsidemargin=10pt \evensidemargin=10pt


==> stuff.tex <==


\noindent
The equivalence $(1) \Leftrightarrow (2)$ is an easy consequence of
To\"en's description~\cite{Toe} of the relationship between dg
functors and kernels. Since we know the cohomology sheaves of
$\cO_{W'}$, the statement $(3)$ is nothing but an algebraic
restatement of $(2)$.  The implications $(3) \Rightarrow (4)
\Rightarrow (5)$ are obvious.  The equivalence $(5) \Leftrightarrow
(6)$ is a dg version of the corresponding statement for schemes,
see~\cite[20.5.12 (iv)]{EGA}, and its proof is identical.  The crucial
part of the proof of Theorem~\ref{thm:mainthm} is the implication $(6)
\Rightarrow (2)$, which will be proved below.


% \paragraph
% The body of the paper consists of four parts.  In the first part we
% prove the ``if'' part of Theorem~\ref{thm:mainthm} and we discuss
% briefly the dependence of the resulting isomorphism on the choice of
% lifting $\bN$ of the normal bundle. The second part is devoted to
% proving the reverse implication.  In Section~\ref{sec:colie} we
% present an alternative point of view on the class $\alpha$ which
% arises from the existence of a natural Lie algebra structure on
% $N[-2]$.  This point of view is similar in spirit (and inspired by)
% Kapranov's work~\cite{Kap}.  We give an explicit example of a closed
% embedding $X\hookrightarrow Y$ where condition $(*)$ is not fulfilled
% in a very brief last section.

% \paragraph
% Throughout the paper we work in slightly greater generality than that
% stated in this introduction.  The subscheme $X$ is only assumed to be
% a local complete intersection, and is not required to be smooth.  All
% schemes are assumed to be over a field $\bbk$ of characteristic zero
% or greater than $\codim X$.

% \paragraph {\bf Acknowledgments.} This paper grew out of conversations
% with Tony Pantev, Lev Rozansky, and Craig Westerland.  The first
% author is a Sloan Research Fellow and he is grateful to the Alfred
% P.~Sloan Foundation for the support.  The second author is supported
% by the National Science Foundation under Grant No.\ DMS-0901224.

% We can achieve this directly as
% follows. Consider the kernels $K_i$ and $K_j$ on $X\times S$ and
% $S\times Y$, respectively, which give rise to the functors $\R
% i_*:\D(X) \ra \D(Y)$ and $\Ld j^*: \D(Y) \ra \D(X)$.  (These are just
% the structure sheaves of the graphs of the morphisms $i$ and $j$.)  It
% is then easy to see that the convolution of these kernels is a kernel
% on $X\times Y$ which has a natural commutative dg algebra structure.
% Hence it defines a dg scheme over $X\times Y$ which is abstractly
% isomorphic to $W'$.  This statement is the dg analogue of the familiar
% fact that if $R_X$ and $R_Y$ are commutative $R_S$-algebras then the
% tensor product $R_X \otimes_{R_S} R_Y$ gives the same answer
% independently of whether we regard $R_X$ and $R_Y$ as symmetric
% $R_S$-bimodules or as $R_X$-$R_S$- and $R_S$-$R_Y$-bimodules.

